Invariant Language Modeling

Large pretrained language models are critical components of modern NLP pipelines. Yet, they suffer from spurious correlations, poor out-of-domain generalization, and biases. Inspired by recent progress in causal machine learning, in particular the invariant risk minimization (IRM) paradigm, we propose invariant language modeling, a framework for learning invariant representations that generalize better across multiple environments. In particular, we adapt a game-theoretic formulation of IRM (IRM-games) to language models, where the invariance emerges from a specific training schedule in which all the environments compete to optimize their own environment-specific loss by updating subsets of the model in a round-robin fashion. We focus on controlled experiments to precisely demonstrate the ability of our method to (i) remove structured noise, (ii) ignore specific spurious correlations without affecting global performance, and (iii) achieve better out-of-domain generalization. These benefits come with a negligible computational overhead compared to standard training, do not require changing the local loss, and can be applied to any language model. We believe this framework is promising to help mitigate spurious correlations and biases in language models.

==> 06_conclusion.tex <==
We introduce invariant language models trained to learn invariant feature representations that generalize across different training environments.
In a series of controlled experiments, we demonstrate the ability of our method to remove structured noise, ignore specific spurious correlations without affecting global performance, and perform better out-of-domain generalization.
These benefits come with a negligible computational overhead compared to standard training, do not require changing the loss, and apply to any language model architecture.
We believe this framework is promising to help alleviate the reliance on spurious correlations and the presence of biases in language models.

==> related_work.tex <==
\section{Related work}

\subsection{OoD}

\begin{itemize}
\item The performance of deep learning models substantially degrades on OOD datasets, even in the face of very small variations of the data generating process \cite{hendrycks2019benchmarking}.
\item Blachard et al. \cite{blanchard2011generalizing} have proposed domain generalization (DG) as a formalism for studying this problem. In DG, the goal is to learn a model using data from from a single or multiple related but distinct training domains, in such a way that the model generalizes well to any OOD testing domain, unknown during training.
\item Recently, the problem of DG has attracted a lot of attention, and has been approached from different facets. 
\item Most of the existing methods fall under the domain alignment \cite{inv_feature_rep, LiGTLT18, adv_inv_features, liu2020causal_semantic_rep, zhao2020entropy_reg}. Motivated by the idea that features that are stable across the training domains should be robust to the unseen testing domains, these methods try to learn domain-invariant representations. The proposed methods differ in the invariance they try to achieve (i.e. what they align) and how they do it (i.e. the distance that they minimize, and how they minimize it).
\item A group of other methods is based on meta-learning \cite{dou2019sem_features, balaji2018metareg, li2018learing_to_generalize}. Following the common meta-learning paradigm, these methods use the training domains to construct disjoint meta-train and meta-test environments. The motivation behind this approach is that it exposes the model to domain shifts during training, which will allow it to generalize better during testing.
% Martin (In case it's useful): While MAML based technique induce a memory and computation bottleneck for the models employed in NLP, it's first-order counterpart FOMAML (https://arxiv.org/pdf/1803.02999.pdf) could potentially provide an alternative for NLP applications...
\item Regularization through data augmentation is commonly used in the training of machine learning models to alleviate overfitting and thereby improve generalization. Based on this idea, \cite{zhou2021feature_noise, zhou2020aug} apply transformations on the original data to simulate a domain shift in training.
\end{itemize}

% Martin (potentially useful reference for data augmentation in NLP): https://aclanthology.org/2021.naacl-main.18.pdf 
%\cite{liu2021counterfactual}

\cite{ye2021oodbench}:
various research areas in OoD (domain generalization, stable learning, IRM) "existing OoD algorithms that outperform empirical risk minimization on one distribution shift usually have limitations on the other distribution shift."" We ask about the language domain.
There is two types of phenomenon: diversity shift and correlation shift.
IRM is focusing on the correlation shift.
Future work can look at invariant representation across language which would be an example of diversity shift.


% Domain generalization via invariant feature representation
% Invariant predictors 
The idea of invariance \cite{inv_feature_rep}, falls into the domain alignment category of approaches for domain generalization. \cite{icc} generalizes the idea in the invariant predictors paper.

** Invariance based on adversarial training principles

% Ya Li et al Domain Generalization via Conditional Invariant Representations. 
\cite{LiGTLT18} adopts different assumptions about what conditionals remain invariant (i.e. learns a feature transformation by minimizing for all classes the variance of class conditional distributions P(X | Y)).

% Masanori Koyama and Shoichiro Yamaguchi. Out-of-distribution generalization with maximal invariant predictor. arXiv:2008.01883, 2020.
\cite{koyama2020oodmax_inv_pred}

% Chang Liu, Xinwei Sun, Jindong Wang, Haoyue Tang, Tao Li, Tao Qin, Wei Chen, and Tie-Yan Liu. Learning causal semantic representation for out-of-distribution prediction. arXiv:2011.01681, 2020.
\cite{liu2020causal_semantic_rep} 

** Regularization tehcniques
% Kamyar Azizzadenesheli, Anqi Liu, Fanny Yang, and Animashree Anandkumar. Regularized learning for domain adaptation under label shifts. In ICLR, 2019.
\cite{azizzadenesheli2019reg_learning} 

% DavidKrueger,EthanCaballero,Joern-HenrikJacobsen,AmyZhang,JonathanBinas,RemiLePriol,and Aaron Courville. Out-of-distribution generalization via risk extrapolation (rex). arXiv:2003.00688, 2020
\cite{kruger2021rex} 

% Haoyue Bai, Rui Sun, Lanqing Hong, Fengwei Zhou, Nanyang Ye, Han-Jia Ye, S-H Gary Chan, and Zhenguo Li. Decaug: Out-of-distribution generalization via decomposed feature representation and semantic augmentation
\cite{bai2021decaug} 

% Recent survey:
% \cite{zhou2021domain} Kaiyang Zhou, Ziwei Liu, Yu Qiao, Tao Xiang, and Chen Change Loy. Domain generalization: A survey. arXiv:2103.02503, 2021
% --> (Martin: Currently going through it) Provides a categorization of the different methodologies for tackling the problem of Domain Generalization(i.e. given training data from a single domain, or multiple distinct but similar domains, learn a model that performs well on a yet unseen target domain), see Table 3 for a summary.

The reason why we chose IRM-games is that most other methods demand computational overhead, for example to perform domain matching, domain variance estimation, estimate mutual information between domains \etc (but in Language modeling, current technology are already compute-intensive and we don't want to increase it more)

The advantage of IRM-games is that it implicitly learns invariant features because of its training dynamics without changing the masked lm loss and without the need to measure any distribution difference/similarities between environments.
IRM-games incurs minimal overhead in training and only few extra-parameters (one lm head per environment) making it a practical implementation of invariant learning for LM.

## Others
\cite{albuquerque2021generalizing} Minimize the discrepancies between pairs of mixtures of domains

\subsection{In language models}

\cite{moradi2021evaluating}
LM suffer from lack of robustness: "The results suggest that language models are sensitive to input perturbations and their performance can decrease even when small changes are introduced."

\cite{wang2021infobert} InfoBERT: Improving Robustness of Language Models from An Information Theoretic Perspective.  ICLR 2021. Boxin Wang, Shuohang Wang, Yu Cheng, Zhe Gan, Ruoxi Jia, Bo Li, Jingjing Liu
Regularization for better robustness in downstream tasks (mostly for textual adversarial attacks)

\cite{tu2020robustness_plm} An Empirical Study on Robustness to Spurious Correlations using Pre-trained Language Models. TACL 2020. Lifu Tu, Garima Lalwani, Spandana Gella, He He

Multi-task learning with data diversity to improve robustness.
This paper also discusses why pretraining help in general -> good motivation for us to work on the language modeling task (best known pretraining task)
--> Has a good related work section that we can use for example of data-augmentation especially. Also some example of techniques that remove the spurious correlation if it is known (but it focuses on NLI and not LM)




\subsection{limitations}

\cite{adv_inv_features} When the domain and the target variable are dependent, there is a trade-off between invariance and accuracy.

% https://arxiv.org/abs/2010.16412: "For other distribution shifts such as those involving confounders or anti-causal variables, however, the two approaches arrive at different asymptotic solutions where IRM is guaranteed to be close to the desired OOD solutions"
